Federated Learning for Semantic Parsing: Task Formulation, Evaluation Setup, New Algorithms

This paper studies a new task of federated learning (FL) for semantic parsing, where multiple clients collaboratively train one global model without sharing their semantic parsing data. By leveraging data from multiple clients, the FL paradigm can be especially beneficial for clients that have little training data to develop a data-hungry neural semantic parser on their own. We propose an evaluation setup to study this task, where we re-purpose widely-used single-domain text-to-SQL datasets as clients to form a realistic heterogeneous FL setting and collaboratively train a global model. As standard FL algorithms suffer from the high client heterogeneity in our realistic setup, we further propose a novel LOss Reduction Adjusted Re-weighting (Lorar) mechanism to mitigate the performance degradation, which adjusts each client's contribution to the global model update based on its training loss reduction during each round. Our intuition is that the larger the loss reduction, the further away the current global model is from the client's local optimum, and the larger weight the client should get. By applying Lorar to three widely adopted FL algorithms (FedAvg, FedOPT and FedProx), we observe that their performance can be improved substantially on average (4%-20% absolute gain under MacroAvg) and that clients with smaller datasets enjoy larger performance gains. In addition, the global model converges faster for almost all the clients.

==> abstract-v1.tex <==
\begin{abstract}
\hs{revised version with comments on overleaf:} Federated learning where multiple clients collaboratively train one global model without sharing their data has been identified as a promising training paradigm. In this paper, we study a new task of cross-silo federated learning (FL) for semantic parsing. \hs{you need to explain what the task is, regardless what specific datasets you used, and why this task is very important.} We propose an evaluation setup to to study this task, where we repurpose eight \ysu{no need to mention the number here} single-domain Text-to-SQL \ysu{text-to-SQL} datasets as eight clients to form the \st{heterogeneous} cross-silo FL setting and collaboratively train a global model. Moreover, we propose a novel \underline {\textbf{LO}}ss \underline{\textbf{R}}eduction \underline{\textbf{A}}djusted \underline{\textbf{R}}e-weighting (\texttt{Lorar}) mechanism\st{FL algorithm}, which can automatically adjust each client's contribution to the global model update during each round\hs{based on what? some short description about how this mechanism works.}. By giving a higher weight to clients that converge more slowly and harder, we implicitly increase the difficulty of the entire training process \hs{this sentence is very important and needs to be more precise} and indirectly enforce the global model toward the direction that takes more care of those clients. \ysu{These two sentences about Lorar are not very precise and convincing. Phrases like ``converge more slowly and harder'', ``implicitly'', ``indirectly enforce'', ``takes more care of'' are vague and weak. Also, this should start with why existing methods are insufficient.} By applying \texttt{Lorar} to \hs{the three widely adopted FL algorithms} (FedAvg, FedOPT and FedProx), we observe that their performance has been improved for almost all the clients with faster convergence, and significant gains can be seen on clients with smaller datasets.  Not correct: \hs{Not sure who put `not correct' here, but Tianshu, please double check this sentence.} In addition, after applying Lorar to FedOPT, almost all clients' performance can exceed their individual finetuning \ysu{Most people probably won't be able to understand the last sentence}.\footnote{Code will be available here: \hs{XX}.}

\end{abstract}

==> background-v1.tex <==
\section{FL for Semantic Parsing}
%{\wl{should we shorten this section?}}
%{\cl{I would suggest we combine Related Work and Background. Tentatively, we can describe details following something like: 1. Text-to-SQL 2) Federated Learning 2a) Training Objective 2b) Training Algorithms (merging the current training procedure and training algorithms, and maybe leave some detailed information such as equations to Section 6.2) 2c) Limitations or Challenges (such as Heterogeneity and lack of benchmark analysis...).}}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/FL2.png}
\caption{An overview of the federated learning procedure.}
\label{illustration of FL}
\end{figure}
\nop{Federated Learning is a training paradigm, which multiple clients collaboratively train a model without sharing their data. There are two realistic types of federated learning: cross-silo setting, and cross-device setting. For the cross-silo setting, clients are large institutions, such as hospitals and companies. In general, they have large computational resources and storage to train and store a large model. And it can also tolerate large communication costs between the server and clients. The number of clients is limited in this setting. For the cross-device setting, clients are small devices like mobile phones and Raspberry Pis. They have limited computational resources and storage and only small communication costs between the server and clients are affordable. It can be a huge number of clients. In our work, we study the cross-silo setting, where each client is a silo that owns its database in its special domain.
}

\subsection{Background}
\hs{shorten this background, especially by being concise.}

\noindent \textbf{Training Objective.} Federated Learning aims to optimize the following objective function:

{\cl{change the first '=' to ':=' or '= min'. Also, should we directly use Eq. (5) instead?}}

\begin{equation}
\begin{aligned}
% a &= b+c\\
% d &= e+f+g
\min\limits_{w} \mathcal{F}(w)&= \mathbbm{E}_{i\sim \mathcal{P}}[\mathcal{L}_i(w)],\\
where \quad \mathcal{L}_i(w)&= \mathbbm{E}_{b\sim \mathcal{D}_i}[f_i(w,b)]. 
\label{eq1}
\end{aligned}
\end{equation}

In \eqref{eq1}, $\mathcal{L}_i (w)$ denotes the local training objective function of the client $i$. $w \in \mathbbm{R}^d$ represents the parameters of the global model, and $\mathcal{P}$ denotes the distribution on the collection of clients $\mathcal{C}$. $b$ denotes each batch of data. The local training loss function $f_i(w,b)$ is often the same across all the clients, while $\mathcal{D}_i$ denotes the distribution of the local client data, which is often different across the clients, capturing the heterogeneity.

%\subsection{Training Procedure} \label{training procedure}
\noindent \textbf{Training Procedure.} Federated learning is an iterative process.
At first, the global server initializes the global model, then there are multiple communication rounds between the server and the clients. Figure \ref{illustration of FL} illustrates this iterative process. In each \textit{communication round}, there are four steps between the server and clients. 1) In round $t$, the server sends the global model $w^t$ to all the clients. 2) After clients receive the global model $w^t$ as the locally initialized model, they start to train it using their own data for multiple epochs and get the accumulated gradients $\Delta w_i^t$. Note that the accumulated gradients for each client are different.
3) The clients send their gradients to the server. 4) The server aggregates the gradients $\Delta w_i^t$ collected from different clients as the formula \eqref{aggregate gradients} shows. 
And then use $t\text{-}th$ round's global model $w^t$ and the aggregated gradients $\Delta w^t$ to update the global model. As the formula \eqref{global model update} shows, $w^{t+1}$ is the global model after the update. The server will send the updated model $w^{t+1}$ to the clients, which also means that the $\text{(}t\text{+}1\text{)}\text{-}th$ round starts. 

The above procedure will repeat until the algorithm converges.

{\cl{pi appears earlier than Eq. 6, let's reorganize Eqs (1)-(6) for concise description}}
\begin{align}
% a &= b+c\\
% d &= e+f+g
\Delta w^t &= p_1 \Delta w^t_1 + p_2 \Delta w^t_2 + ... + p_N \Delta w^t_N
\label{aggregate gradients} \\
w^{t+1} &= w^t - \Delta w^t 
\label{global model update}
\end{align}

%\subsection{FL Algorithms}
\noindent \textbf{FL Algorithms.} We explore three popular FL algorithms: FedAvg, FedOPT, and FedProx in our text-to-SQL problem.

\textit{Federated Averaging (FedAvg)} \cite{mcmahan2017communication} uses stochastic gradient descent (SGD) as the local training optimizer to optimize the training procedure we mentioned in section \ref{training procedure} and uses the same learning rate and local training epochs for all the clients.

\textit{FedOPT} \cite{reddi2020adaptive} is a generalized version of FedAvg. It has a special design to treat the negative aggregated gradients "$-\Delta w^t$ on the server as a pseudo-gradient. Thus different adaptive optimizers can be used to update the server due to the benefit of such a pseudo-gradient. For the client side, FedOPT also allows for more powerful adaptive optimizers to optimize the local training stage.

\textit{FedProx} \cite{li2020federated} tries to tackle the statistical heterogeneity issue by adding an L2 regularization term, which constrains the local model to be closer to the initialized local model(i.e., the global model) during each round for stable training.

Both FedAvg and FedOPT optimize the local training objective $f_i(w,b)$.
% \begin{align}
% f_i(w,b) = l_i(w,b) \label{fedavg/fedopt}
% % f_i(w,b) &= l_i(w,b)+\frac{\mu}{2}\Vert w-w^t\Vert^2 \label{fedprox}    
% \end{align}
For FedProx, instead of just optimizing $f_i(w,b)$, it uses the local optimizer to optimize the following local objective \eqref{fedprox}. $\mu$ is the hyperparameter, and $w^t$ is the initial local model(i.e., the global model) during $t \text{-}th$ round. Note $w^t$ varies during each round.
\begin{align}
% f_i(w,b) &= f_i(w,b) \label{fedavg/fedopt}\\
\min\limits_{w} h_i(w,b,w^t) = f_i(w,b)+\frac{\mu}{2}\Vert w-w^t\Vert^2 \label{fedprox}    
\end{align}

For the cross-silo setting which all the clients participate in the training for each round, all these three algorithms minimize \eqref{eq1} which is equivalent to \eqref{equivalent}: 
\begin{align}
\min\limits_{w} \mathcal{F}(w) = \sum\nolimits_{i=1}^N p_i \mathcal{L}_i (w)
\label {equivalent}   
\end{align}
and they define $p_i$ as the training size proportion \eqref{size proportion}. $\left|\mathcal{D}^i\right|$ is the training size of the client $i$. $N$ denotes the number of clients.
\begin{align}
p_i = \left|\mathcal{D}^i\right|/\sum\nolimits_{i=1}^N \left|\mathcal{D}^i\right|
\label {size proportion}   
\end{align}

% $\min\limits_{w} f(w) = p_1 L_1 (w)+p_2 L_2, which  (w) + ... + p_N L_N (w)$ \\

\begin{table*}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{0.11\linewidth}|c||ccc||cccccccc}
\hline
\text{} & \text{} & \text{} & \text{} & \text{} & \text{Questions} & \multicolumn{2}{c}{Unique tables} & \multicolumn{2}{c}{SELECTs} & \multicolumn{2}{c}{Nesting}\\
\text{} & \text{Domain} & \text{Train} & \text{Dev} & \text{Test} & \text{/ unique query} & \multicolumn{2}{c}{/ query} & \multicolumn{2}{c}{/ query} & \multicolumn{2}{c}{Depth} \\
\text{} & \text{} & \text{} & \text{} & \text{} & \text{} & \text{$\mu$} & \text{Max} & \text{$\mu$} & \text{Max} & \text{$\mu$} & \text{Max} \\
\hline
Advising & Course Infomation & 2629 & 229 & 573 & 21.7 & 3.0 & 9 & 1.23 & 6 & 1.18 & 4\\
ATIS & Flight Booking & 4347 & 486 & 447 & 5.6 & 3.8 & 12 & 1.79 & 8 & 1.39 & 8 \\
GeoQuery & US Geography & 549 & 49 & 279 & 3.6 & 1.1 & 4 & 1.77 & 8 & 2.03 & 7 \\
Restaurants & Restaurants/Food& 228 & 76 & 74 & 16.4 & 2.3 & 4 & 1.17 & 2 & 1.17 & 2 \\
Scholar & Academic Publication& 499 & 100 & 218 & 4.2 & 3.2 & 6 & 1.02 & 2 & 1.02 & 2 \\
\hdashline
Academic & Microsoft Academic& 120 & 38 & 38 & 1.1 & 3 & 6 & 1.04 & 3 & 1.04 & 2 \\
IMDB & Internet Movie & 78 & 26 & 26 & 1.5 & 1.9 & 5 & 1.01 & 2 & 1.01 & 2 \\
Yelp & Yelp Website& 78 & 26 & 24 & 1.2 & 2 & 4 & 1 & 1 & 1 & 1\\
\hline
\end{tabular}}
\caption{\label{data statistics}
Statistics for Heterogeneous text-to-SQL datasets. Datasets in the first group are human-generated from NLP community, while datasets in the second group are human-generated from DB community.}
\end{table*}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/restaurant_db3.png}
\caption{An overview of the text-to-SQL task. }
\label{text2sql}
\end{figure}


==> intro-v1.tex <==
\section{Introduction{\wl{as we discussed before, should we include motivating example here?}}}
{\cl{The story line should be something like: we first talk about text2SQL tasks, then introduce its challenges in practical applications due to data privacy, then we introduce FL, however directly applying FL to text2SQL are limited due to heterogeneity (existing work are either less practical or lack comprehensive analysis), so we propose our work to overcome these limitations where we 1) formulate the cross-silo federated learning setting for text2SQL task based on a large language model, 2) setup practical evaluation benchmark 3) develop new algorithm 4) extensively verify effectiveness of our method (please see more details below)}}
% Main point: 

% Draw a figure for fl and text2sql 
% change FedOPT to upper case 
% Data description

% Cross-silo setting vs cross-device setting. Cross-silo setting is what we do here.

% Bidirectional explanation: fl helps text2sql, text2sql provides a more realistic bencmark for studying fl. Though fl do help us to get one more generalization model, it exposes an issue  of current algo, which is bad performance on small datasets. (xx work also work on similar problem, but they 1) lack of realistic benchmark, existing mainly focus on using Dirichlet distribution to split well-defined datasets to non-iid like cifar 10 (eg xx) or use transformer to skew generation sentence (fednlp). However, the disadvantages for these two 2) more on image classfication tasks, rather than complex logic form generation task 3) local model, current work do exp are small model, and local optimizer is not specific. We use T5 (large pretrained langage model, and use the optimizer for T5) 4) We proposes a simple but effective method: loss change adjusted re-weighting to address this issue. Complementary to current popular algorthms(change optimizer on global or local or add regularizer on local)(cite paper, also gradient similarity) our exps shows very promising results, which combined it with fedopt, the performance on small datasets improve a lot, without affect other clients' performance. For Fedavg and FedProx, 

% text2sql: lack of realistic data (hard to annotate for both grammatically and semantically correct, hard to annotate privacy needs
% selling point: 1>benefit clients with fewer datasets, 2>for large data, their data themselves is enough to train a neural model to serve themselves. But still, by other clients participates, only one global model has gained better generalization ability, and may have better performance on additional data added later compared with finetuning.

% The motivation to build a text-to-sql fl system. lack of database data. FL to protect data of different organizations. Current work work on synthetic data, more on image classification tasks, or try to split existing dataset based on class labels. 

% \hs{In this paper, we study federated learning for Text-to-SQL.}

% \hs{The logic in the following 2 paragraphs is OK. They just need to be condensed and polished}

% Natural language interfaces that allow users to query data and invoke services without programming have been identified as a key application of semantic parsing \cite{}.
Neural semantic parsers have achieved remarkable performance in translating natural language questions into logical forms \ysu{I won't use the phrase ``logical forms''. It's not accurate. Use meaning representations or programs.} \cite{}{\cl{add refs}}. As one fundamental task \ysu{I won't call it fundamental. maybe popular. Also, as the title suggests, the scope of this paper is for semantic parsing in genral, with text-to-SQL as an example and evaluation setting. So the intro here is getting too specific too soon.} of semantic parsing, text-to-SQL enables users to query databases by directly asking questions without writing SQL. However, some institutions only have limited data, which makes it hard for them to build their own neural natural language interfaces by themselves. Collecting data on such cases is a big challenge due to two reasons. On the one hand, data owners such as hospitals, financial institutions, or legal firms are unwilling to share their data with others since databases and questions always contain private user information. On the other hand, it's hard to annotate logical form generation data on a large scale, as it requires the annotators to master the basic knowledge of both the syntactic and semantic meaning of the logical forms {\cl{Let's reorganize the above two limitations especially the second one. The first limitation can motivate the adoption of FL. Not sure whether it is the same case for the second limitation as well...}}. \ysu{the second limitation is also part of the motivation. If data collection is super easy, we wouldn't need to resort to FL to hopefully benefit from others' data. But agree it needs to be made more clear.}

\hs{Revised Pg. 1: Semantic parsing aims to translate natural language utterances into formal meaning representations such as SQL queries and API calls and has numerous applications in building natural language interfaces that enable users to query data and invoke services without programming \cite{XX} . Neural semantic parsers have achieved remarkable performance in recent years \cite{XX}. However, they are data-hungry; bootstrapping a neural semantic parser by annotating data on a large scale can be very challenging for many institutions, as it requires the annotators to have intimate knowledge about formal programs.  One natural thought is to leverage data from different institutions and train a unified model that can be used for all applications. However, in practice, institutions such as hospitals, banks, and legal firms are prohibited from sharing their data with others, due to privacy concerns. Therefore, for institutions that only have very limited data, it is extremely hard to build their own neural semantic parsers.
}
% In reality, different institutions such as hospitals, financial institutions, or legal firms have their own private databases in their special domains. However, some institutions only have limited data, which increases the difficulty to build a neural natural language interface by themselves. Unlike other general tasks in NLP, the databases and corresponding questions for the text-to-SQL task often contain important realistic user information, thus the data owners are unwilling to share their data with others to train the model, due to privacy concerns. On the other hand, it's hard to annotate data on a large scale, especially in the logical form(SQL) generation scenario, since it requires annotators to master the basic knowledge of both the semantic and syntactic meaning of the logical form.

% Federated learning (FL) is a popular training paradigm in which multiple clients can collaboratively train a global model without exchanging their own data. In the federated learning setting, each client just needs to train the model locally and send their local models to the server without exposing their data to others. Then the server aggregates different local models collected from different clients and sends the new updated global model to clients. This is an iterative process that takes multiple communication rounds between the server and clients, in order to get a good global model to satisfy different clients. By exploiting the scattered data from different institutions, all institutions can finally get a global model which has better generalization ability to help improve the performance on their own, especially beneficial for those institutions who have insufficient data to build their own neural models.

Federated learning (FL) is a popular training paradigm in which multiple clients can collaboratively train a global model without exchanging their own data. In our work, we propose to use FL to solve the challenge above {\cl{see previous comment}}. By exploiting the scattered data from different institutions, all institutions \hs{this is not true, right?} can finally get a global model which has better generalization ability to help improve the performance on their own, especially beneficial for those institutions who have insufficient data to build their own neural models.

\hs{Revised Pg. 2: Federated learning (FL) \cite{XX} has turned out to be a popular training paradigm where multiple clients can collaboratively train a global model without exchanging their own data. In this paper, we study a new task of federated learning for semantic parsing. Through FL on the data scattered on different clients (e.g., institutions), we aim to obtain a global model that works well for all clients, especially those that have insufficient data to build their own neural models.}

\hs{Revised Pg. 3: Towards that end, we propose an evaluation setup by re-purposing existing datasets that are widely adopted for text-to-SQL, such as ATIS \cite{XX} and GeoQuery \cite{XX}. These datasets demonstrate great heterogeneity, in terms of dataset sizes, language usage, database structures, and SQL styles, as they were created by different researchers, at different times, and for different purposes. Therefore, we use this collection to simulate a realistic scenario where eight clients with very different data participate in the FL paradigm to jointly train a neural semantic parser.}

{\cl{However, directly applying FL to text2SQL are limited due to heterogeneity (existing work are either less practical or lack comprehensive analysis)}}
As one of the biggest challenges in FL, heterogeneity always leads to performance deterioration when the data distributions and data sizes of different clients are different. A myriad of methods \cite{li2020federated, li2021fedbn, shoham2019overcoming, t2020personalized} incorporate extra proximal terms to handle the data in label distribution skew \cite{kairouz2021advances}. However, they either use synthetic data \cite{li2020federated} or split classification datasets based on Dirichlet distribution \cite{lin2021fednlp} to simulate the non-i.i.d federated learning setting, which lacks a more realistic benchmark to evaluate their performance of the cross-silo FL \hs{this term is foreign to ACL people. we need to clarify what it is.}. Moreover, only limited work has studied federated learning on more complex tasks such as generation tasks \cite{lin2021fednlp}. Even \citealp{lin2021fednlp} \hs{I think we should leave these nuances in related work...}tries to use MRQA \ysu{magic word without definition or reference} to simulate the cross-silo heterogeneous setting, they just simply show the overall performance of the global model, which lacks the analysis of how the final global model performs on each client. {\cl{I assume we want to focus on challenges of directly applying FL to text2SQL, therefore applying large-scale model is not suitable here. We can integrate it to the next paragraph...BTW, we need to rethink why we want to adopt a large-scale model. The following reason of convenience is not that strong... Maybe we want to say: large pre-trained models have achieved success thus can be leveraged to provide even more improvement for our setting... }} Furthermore, as the large pre-trained models have achieved surprising \ysu{wouldn't call it surprising} success, it's more convenient \ysu{won't use words like convenient in professional writing; it's weak} for different clients to collaboratively train the same unified model without considering the special model design for each client. But the study for the realistic large model-based cross-silo federated learning is still limited. 


% \hs{we should get to our contributions faster. the above discussions could be more concise and some may be moved to related work.} 
In our work, we repurpose eight single-domain text-to-SQL datasets as eight clients to study cross-silo federated learning. The datasets and tasks we study are more realistic and more complex, and we also use T5-base, a large and powerful unified pre-trained language model as our backbone model. As existing federated learning algorithms perform badly on our benchmark and it's hard for some clients to converge, also as we observe that the training loss reduction is a good indicator to show how worse the global model is away from the local optima of each client, \ysu{generally this is a rather weak way to motivate your method. It reads like, okay we tried existing methods and somehow they didn't work so we propose some way to put a ``patch" on them that's hopefully better. A better way to motivate would be to clearly discuss your new insights about why existing methods are insufficient (e.g., why unique properties of your realistic setting cause that), and why that motivate you to come up with the new approach, and why intuitively the new approach would work better.} we propose to use training loss reduction as an additional factor to adaptively control how much each client should contribute to the global model update during each round. Our proposed simple yet effective method achieves the best in both the model performance and the training convergence speed compared with FedAvg, FedOPT and FedProx on our benchmark.

\hs{Revised Pg. 4: Heterogeneity, where the data distributions and dataset sizes on different clients are different, is recognized as one of the biggest challenges in FL \cite{XX}.  Existing work either uses synthetic data \cite{li2020federated} or splits a dataset based on Dirichlet distribution \cite{lin2021fednlp} to simulate the non-i.i.d federated learning setting, while we propose a more realistic setup to study this setting for semantic parsing. Pre-trained language models such as T5 have been shown as a powerful unified model for various semantic parsing tasks, which saves us the efforts for client-specific model designs. We adopt T5-base as our backbone semantic parser in the FL paradigm, and conduct extensive experiments and analysis using three widely-adopted FL algorithms (X Y Z).} 

\hs{Revised Pg. 5: Furthermore, we propose a novel re-weighting mechanism for combining the gradient updates from each client during the global model update. The high-level idea is shown in Figure XX. Our intuition is that [for each client, the training loss reduction in each round can be a good indicator of how far the global model is away from the local optima of that client...]. We formulate this intuition as a re-weighting factor to adjust how much each client should contribute to the global model update during each round. Our proposed mechanism can be applied to all the three FL algorithms and experiments show that it can substantially improve both their parsing performance and their convergence speed, despite being very simple.
}{\cl{Motivating Example: as can be seen in Figure~{fig:example}, the training loss ..... After applying our method, the training loss....}}

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{figures/motivation_example.png}
\caption{\cl{Let's add two more figures of the new training losses after applying the new method. \ysu{this comes too late. It needs to be on parge 1 and referenced multiple times in the intro}} \hs{I think it's ok to put it on page 2. This isn't the contribution that is worth the most highlight.}}
\label{motivation_example}
\end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=1.45in]{figures/motivation_example.png}
% \caption{} Training loss of two clients: Restaurants and Yelp. The fluctuation shows how far the global model is away from the local client's optima.}
% \label{fig:example}
% \end{figure}
\hs{Revised summary: In summary, our main contributions are:
\begin{itemize}
\item [$\bullet$]To the best of our knowledge, we are the first to study federated learning for semantic parsing, a promising paradigm for multiple institutions to collaboratively build natural language interfaces without data sharing, which is especially beneficial for institutions with little training data. %And we use T5-base, a large pre-trained language model to unify all clients.
\item [$\bullet$]We propose an evaluation setup to simulate a realistic heterogeneous FL setting where different participating institutions have very different data. We re-purpose eight single-domain datasets for text-to-SQL as eight clients, which demonstrate high heterogeneity in terms of dataset sizes, language usage, database structures and SQL styles. %This enables us to test how current FL algorithms perform on a realistic heterogeneous FL setting.
\item [$\bullet$]We propose a novel re-weighting mechanism, which uses the loss reduction of each client to adjust its contribution to the global model update during each round. Experiments show that our re-weighting mechanism can substantially improve the model performance of existing FL algorithms on average, and clients with smaller training data observe larger performance gains. %Also, by applying our proposed algorithm to FedOPT, the global model can outperform individual finetuning on clients with smaller training data (i.e., ).   
\end{itemize}
}

==> problem_formulation-v1.tex <==
\section{Problem Formulation {\wl{let's plan to reorganize Sections 4-6}}}
{\cl{let's elaborate more on this task formulation to highlight our contribution here. Current description is more about general text2SQL task itself, we should start discussing the cross-silo federated learning setting of text2SQL task at the very beginning.}}
Text-to-SQL is a task in which the model generates the logical form (SQL) $Y$ given natural language question $Q$ and database schema $\mathcal{S=<C,T>}$. It aims to automatically translate the question in human language to SQL so as to query the database to get the answer to the question. Here the question $Q = q_1,q_2,...,q_{|Q|}$ is a sequence of words. Database schema $\mathcal{S}$ contains multiple tables $t_i$ with each table containing multiple columns $c_{i,j}$. We concatenate the question token $q_k$ with the database schema $\mathcal{S}$ as the model input, to generate the output SQL token $y_1, y_2,...,y_{|Y|}$.

In our work, all the clients are playing a role as a different "institution" that contains its own private database and questions. These clients collaboratively train the global model. A deeper description of these clients is in section \ref{benchmark}.
